Managing caching strategies for stream reasoning with reinforcement learning

Efficient decision-making over continuously changing data is essential for many application domains such as cyber-physical systems, industry digitalization, etc. Modern stream reasoning frameworks allow one to model and solve various real-world problems using incremental and continuous evaluation of programs as new data arrives in the stream. Applied techniques use, e.g., Datalog-like materialization or truth maintenance algorithms to avoid costly re-computations, thus ensuring low latency and high throughput of a stream reasoner. However, the expressiveness of existing approaches is quite limited and, e.g., they cannot be used to encode problems with constraints, which often appear in practice. In this paper, we suggest a novel approach that uses the Conflict-Driven Constraint Learning (CDCL) to efficiently update legacy solutions by using intelligent management of learned constraints. In particular, we study the applicability of reinforcement learning to continuously assess the utility of learned constraints computed in previous invocations of the solving algorithm for the current one. Evaluations conducted on real-world reconfiguration problems show that providing a CDCL algorithm with relevant learned constraints from previous iterations results in significant performance improvements of the algorithm in stream reasoning scenarios. Under consideration for acceptance in TPLP.

==> impl.tex <==
\section{Implementation}
\label{sec:solver}

\begin{figure}[h]
\includegraphics[height=85mm]{figures/schematic.pdf}
\caption{Schematic overview of the distributed system and a solver component.}
\end{figure}

\begin{algorithm}
  \SetKwFunction{ProcessAssumptions}{UpdateAssumptions}
  \SetKwInOut{AlgoInput}{input}\SetKwInOut{AlgoOutput}{output}\SetKwInOut{AlgoPersist}{persistent}
  \SetKw{Break}{break}

  \AlgoInput{ delta from stream partitioned into $L^{+}$ and $L^{-}$}
  \AlgoOutput{an answer set $I$ or $\mathit{incoherent}$}
  \AlgoPersist{clause set $C$ with values $V$, assumptions vector $A_{t}$}

  $A_t \gets $ \ProcessAssumptions($L^{+}$, $L^{-}$, $A_{t-1}$)\;

  \For{clause $c_{i} \in C$, ordered by value $v_{i} \in V$}{ %
    \eIf{$i < k$}{
      thaw clause $c_{i}$ in solver
    }{
      freeze clause $c_{i}$ in solver
    }

    \If{$i > n$}{
      delete clause $c_{i}$ in solver
    }
  }

  $I \gets$ call solver with assumptions $A_{t}$, adding any learned clauses to $C$\;

  \For{clause $c_{i} \in C$}{
    $\rho \gets$ reward for clause $c_{i}$\;
    $v_{i} \gets v_{i} + \alpha (\rho - v_{i})$\;
  }

  \Return{$I$}

  \caption{ProcessNewInput\label{algo:management}}
\end{algorithm}

\kstodo{describe settings of the solver, reward functions, heuristics
Learning stationary distribution}

LBD is modified only for conflicts that were involved in the
computations for the current instance. Conflicts in LBD values that were
stored in the solver remain unchanged unless a conflict is reused
during the current search iteration. In this way, the quality of
conflicts from the previous solving runs is compared to the quality of
conflicts in the current run.

It might get stuck.

Learning non-stationary case
